Emptiness and Universality Problems in Timed Automata with Positive Frequency

The languages of infinite timed words accepted by timed automata are traditionally defined using Buchi-like conditions. These acceptance conditions focus on the set of locations visited infinitely often along a run, but completely ignore quantitative timing aspects. In this paper we propose a natural quantitative semantics for timed automata based on the so-called frequency, which measures the proportion of time spent in the accepting locations. We study various properties of timed languages accepted with positive frequency, and in particular the emptiness and universality problems.

==> cases.tex <==
\fbox{Ci-dessous quelques notations a mettre a un endroit adequat et
  peut etre a modifier!!!}

Given $\rho=s_0\xrightarrow{\tau_1,a_1} s_1\cdots
\xrightarrow{\tau_k,a_k} s_{k} \cdots$ a run of $\A$, we
denote by $\rho_{\le n}$ its prefix of length $n$, i.e.  $\rho_{\le n} =
s_0 \xrightarrow{\tau_1,a_1} s_1\cdots
\xrightarrow{\tau_n,a_n} s_{n}$.

\fbox{Definir (abusivement) $\freq{\rho_{\le n}} $ et $\Rat{\pi_{\le n}}$}

\fbox{Dans la suite, je suppose travailler avec les regions
  'adequates' une horloge}

\fbox{Je suppose aussi transitivité dans le corner-point pondere...}

\fbox{Cela induit peut être une non unicité des dilatations/contractions... mais unique a transitivite pres...}

\begin{lemma}\label{lem-cases}
  Let $\A$ be a timed automaton, $\rho$ be a run of $\A$, and $\pi_n$
  be the dilatation of $\rho_{\le n}$ (for $n \in \IN$). For all $n \in
  \IN$,
$\text{if } \freq{\rho_{\le n}} = \frac{c_n}{r_n} \text{ and } \Rat{\pi_{\le n}} = \frac{C_n}{R_n} \text{ then } C_n \ge c_n \text{ and } (R_n-C_n) \le (r_{n} - c_{n})$.
\end{lemma}

\begin{proof}
  The proof is by induction on $n$. \fbox{Smart idea for the base or
    many cases to do as well???}

  Let us now assume that the lemma holds for $n$ and let us prove it
  for $n+1$. We have that $\rho_{\le n+1} =
  s_0 \xrightarrow{\tau_1,a_1} s_1\cdots
  \xrightarrow{\tau_n,a_n} s_{n}
  \xrightarrow{\tau_{n+1},a_{n+1}} s_{n+1}$. We will have
  to distinguish several cases depending of the last transition of
  $\rho_{\le n+1}$. To ease the notation we will denote $s_n$
  (resp. $s_n+1$) by $s=(\ell,v)$ (resp. $s=(\ell',v')$) and
  $\tau_{n+1}$ (resp. $a_{n+1}$) by $\tau$ (resp. $a$). We also denote
  $g$ the guard of the last transition and $R$ (resp. $R'$) the region
  containing $v$ (resp. $v'$). 
  \begin{enumerate}
  \item \label{cas1} Assume that $\fract{v}=0$ \fbox{A definir???},
    $\ell \in F$, and there is no equality in $g$. In this case, we
    can write $\tau=\tau_0 + \tau_1$ with $\tau_0 \in \IN$ and $0<
    \tau_1 <1$. Assuming that $v+\tau \not\in \bot$, by definition of
    the dilatation, we have that $\pi_{\le n+1} = \pi_{\le n}
    \xrightarrow{\tau_0/\tau_0} (\ell,R,\gauche) \xrightarrow{1/1}
    (\ell,R,\droite) \xrightarrow{0/0} (\ell',R',\alpha')$. \fbox{OK?}


    \fbox{Mes notations jouent sur le fait que je suppose $\A_{cp}^F$
      transitif}

    \fbox{La notation est aussi un peu abusive car elle ne tient pas
      compte du cas $\tau_0=0$}

    We thus have that $C_{n+1} = C_n + \tau_0 + 1$, $c_{n+1} = c_n +
    \tau_0 + \tau_1$, $R_{n+1} = R_n + \tau_0 + 1$ and $r_{n+1} = r_n
    + \tau_0 + \tau_1$. In particular, we have that that $C_{n+1} \ge
    c_{n+1}$, since $C_{n} \ge c_{n}$ (by induction hypothesis) and
    $\tau_1<1$. Moreover we have that $(R_{n+1}-C_{n+1}) \le (r_{n} -
    c_{n})$ since $(R_{n+1}-C_{n+1}) = (R_{n}-C_{n})$,
    $(r_{n+1}-c_{n+1}) = (r_{n}-c_{n})$ and $(R_{n}-C_{n}) \le (r_{n}
    - c_{n})$ (by induction hypothesis). The case where $v+\tau \in
    \bot$ is handled similarly. \fbox{OK?}

  \item Assume that $\fract{v}=0$, $\ell \not\in F$, and there is no
    equality in $g$. In this case, we can write $\tau=\tau_0 + \tau_1$
    with $\tau_0 \in \IN$ and $0< \tau_1 <1$. Assuming that $v+\tau
    \not\in \bot$, by definition of the dilatation, we have that
    $\pi_{\le n+1} = \pi_{\le n} \xrightarrow{\tau_0/\tau_0}
    (\ell,R,\gauche) \xrightarrow{0/0} (\ell',R',\alpha')$.  We thus
    have that $C_{n+1} = C_n + \tau_0 $, $c_{n+1} = c_n + \tau_0 $,
    $R_{n+1} = R_n + \tau_0 $ and $r_{n+1} = r_n + \tau_0 $. As in the
    previous case, one can deduce the desired result from this
    equalities. \fbox{OK?}  The case where $v+\tau \in \bot$ is
    handled similarly. \fbox{OK?}

  \item Assume that $\fract{v}=0$, $\ell \in F$, and there is an
    equality in $g$. In this case, we have that $\tau \in \IN$.  By
    definition of the dilatation, $\pi_{\le n+1} = \pi_{\le n}
    \xrightarrow{\tau/\tau} (\ell,\{c\},\alpha \fbox{Notation OK?})
    \xrightarrow{0/0} (\ell',R',\alpha')$.  We thus have that $C_{n+1}
    = C_n + \tau$, $c_{n+1} = c_n + \tau$, $R_{n+1} = R_n + \tau$ and
    $r_{n+1} = r_n + \tau$. As in the previous case, one can deduce
    the desired result from this equalities. \fbox{OK?}

  \item Assume that $\fract{v}=0$, $\ell \not\in F$, and there is an
    equality in $g$. In this case, we have that $\tau \in \IN$.  By
    definition of the dilatation, $\pi_{\le n+1} = \pi_{\le n}
    \xrightarrow{0/\tau} (\ell,\{c\},\alpha \fbox{Notation OK?})
    \xrightarrow{0/0} (\ell',R',\alpha')$.  We thus have that $C_{n+1}
    = C_n$, $c_{n+1} = c_n$, $R_{n+1} = R_n + \tau$ and $r_{n+1} = r_n
    + \tau$. As in the previous case, one can deduce the desired
    result from this equalities. \fbox{OK?}

  \item \fbox{Cas du garde $x= 0$ Necessaire???}
    
  \item Assume that $\fract{v} \ne 0$, $\ell \in F$, and there is no
    equality in $g$. In this case, we can write $\tau = \tau_0 +
    \tau_1$ with $\tau_0 \in \IN$ and $0 \le \tau_1 <1$. Notice that
    $\tau_1$ can be equal to zero but we know that $v + \tau \not\in
    \IN$.  Assuming that $v+\tau \not\in \bot$, by definition of the
    dilatation, we have that $\pi_{\le n+1} = \pi_{\le n}
    \xrightarrow{\tau_0/\tau_0} (\ell,R,\gauche) \xrightarrow{1/1}
    (\ell,R,\droite) \xrightarrow{0/0} (\ell',R',\alpha')$. We are
    thus in a situation similar to case~\ref{cas1}. \fbox{OK?}

  \item Assume that $\fract{v} \ne 0$, $\ell \in F$, and there is an
    equality in $g$. \fbox{A DISCUTER}

  \item \fbox{A DISCUTER}

    
  \end{enumerate}

\end{proof}

==> sec-conseq.tex <==
\subsection{Deterministic timed automata}\label{section:decid}

\fbox{TB: On doit commencer par une remarque sur les regions one clock
  pour la complexite...}

Theorem~\ref{th:setfreq} immediately yields the decidability of the
emptiness problem for the frequency-language of single-clock timed
automata. Indeed the bounds of the set of frequencies are computable,
and one can decide whether they are reached. Hence, it is
straightforward to decide whether some execution has positive
frequency.
\begin{corollary}
  The emptiness problem of frequency languages is
  NLOGSPACE-Complete\nat{check complexity} for single clock timed
  automata.
\end{corollary}

Moreover, for the restricted class of deterministic timed automata,
considering all words exactly amounts to considering all
executions. Thanks to Theorem~\ref{th:setfreq}, one can decide, in
this case, whether the unique execution on every word has a positive
frequency:
\begin{corollary}
  The universality problem of frequency languages is
  NLOGSPACE-Complete\nat{check also here} for single clock timed
  automata.
\end{corollary}

\begin{remark}
  In the two latter corollaries, we consider the emptiness and
  universality problem for the languages of timed automata under
  frequency-acceptance with threshold $0$. Note that they would extend
  to any threshold $\lambda \in (0,1)$.
\end{remark}

